Bandit algorithms for real-time data capture on large social medias

We study the problem of real time data capture on social media. Due to the different limitations imposed by those media, but also to the very large amount of information, it is impossible to collect all the data produced by social networks such as Twitter. Therefore, to be able to gather enough relevant information related to a predefined need, it is necessary to focus on a subset of the information sources. In this work, we focus on user-centered data capture and consider each account of a social network as a source that can be listened to at each iteration of a data capture process, in order to collect the corresponding produced contents. This process, whose aim is to maximize the quality of the information gathered, is constrained by the number of users that can be monitored simultaneously. The problem of selecting a subset of accounts to listen to over time is a sequential decision problem under constraints, which we formalize as a bandit problem with multiple selections. Therefore, we propose several bandit models to identify the most relevant users in real time. First, we study of the case of the stochastic bandit, in which each user corresponds to a stationary distribution. Then, we introduce two contextual bandit models, one stationary and the other non stationary, in which the utility of each user can be estimated by assuming some underlying structure in the reward space. The first approach introduces the notion of profile, which corresponds to the average behavior of a user. The second approach takes into account the activity of a user in order to predict his future behavior. Finally, we are interested in models that are able to tackle complex temporal dependencies between users, with the use of a latent space within which the information transits from one iteration to the other. Each of the proposed approaches is validated on both artificial and real datasets.

==> Chapitre3Old.tex <==
\chapter{Modèle contextuel}
	\minitoc
	\newpage
    
    
\label{ModeleContextuelVariable}

La modélisation d'un profil pour chaque utilisateur associé à une hypothèse linéarité nous a permis d'améliorer considérablement les performances de notre processus de collecte dans le chapitre précédent. En effet grâce à la présence d'un paramètre de régression commun à tous les utilisateurs, nous avons montré qu'il est possible de mutualiser l'apprentissage, permettant ainsi une exploration plus intelligente de l'espace des utilisateurs. Cependant, l’hypothèse majeure nous ayant permis de dériver l'algorithme associé était la stationnarité des profils. Concrètement, étant donné que nous avons choisi d'utiliser le "message moyen" - à une transformation LDA près - comme profil, cela signifie que les utilisateurs n'ont tendance à poster qu'un seul type de message. Cette hypothèse peut être discutée, car il est possible que certains utilisateurs soient actifs sur plusieurs sujets complètement différents selon par exemple le moment de la journée. Dans ce cas, le modèle précédent n'est plus valide, car ne prenant pas en compte cette éventualité, qui pour être clair correspondrait à un changement de profil. Pour pallier cette faiblesse, nous proposons dans ce chapitre de modéliser des profils d'utilisateurs variables au cours du temps. Nous traitons ce problème comme un bandit contextuel prenant en comptes les contraintes associées à notre tâche, à savoir l'impossibilité d'observer tous les contextes. Dans cette optique nous dérivons deux algorithmes que nous expérimenterons sur des données réelles et artificielles.


 

\section{Modèle}

Dans cette section, nous formalisons le modèle mathématique de bandit contextuel ainsi que les hypothèses correspondantes.  On suppose qu'il existe un vecteur inconnu permettant d'estimer l'espérance de la récompense que l'on peut observer pour chaque action en fonction de son vecteur de contexte. On se place ici dans le cas où le nombre d'actions $K$ est fini. Ainsi, à chaque pas de temps $t\in \left\{1,..,T\right\}$, chaque action $i\in \left\{1,..,K\right\} =\mathcal{K}$ révèle un vecteur de contexte noté $x_{i,t} \in \mathbb{R}^{d}$ et l'agent sélectionne un ensemble $\mathcal{K}_{t}$ de $k<K$ actions pour lesquels il reçoit les récompenses associées, son but étant toujours de maximiser la somme des récompenses cumulées au cours du temps. L'hypothèse classique \cite{banditThompsonCtxtPreuve} permettant de lier contexte et récompense est la suivante :
 
 
 \begin{equation}
 \exists \beta \in \mathbb{R}^{d} \text{ tel que } \forall t \in \left\{1,..,T\right\}, \forall i \in \left\{1,..,K\right\}: \mathbb{E}[r_{i,t}|x_{i,t}]=x_{i,t}^{\top}\beta
 \end{equation}

Dans notre cas, le contexte $x_{i,t}$ de chaque utilisateur $i$ à chaque instant $t$ correspond au contenu publié dans la fenêtre de temps $t-1$. Contrairement au chapitre précédent, on utilise directement l'échantillon révélé par un utilisateur et non pas une moyenne. On remarque que dans ce cas, si un utilisateur est inactif au temps $t-1$, c'est à dire possède un vecteur de contexte nul, son espérance sera forcément égale à zéro. Or nous souhaitons éviter cette situation, car un utilisateur peut être actif de façon ponctuelle à un instant donné sans l'avoir été au temps précédent. Ainsi, afin de modéliser la qualité intrinsèque de chaque utilisateur, nous introduisons également un terme de biais $\theta_{i} \in \mathbb{R}$ pour chaque compte $i$. L'hypothèse de travail devient la suivante :

\begin{equation}
\exists \beta \in \mathbb{R}^{d},  \exists \left(\theta_{1},...,\theta_{K}\right) \in \mathbb{R}^{K} \text{ tels que }\forall t \in \left\{1,..,T\right\}, \forall i \in \left\{1,..,K\right\}: \mathbb{E}[r_{i,t}|x_{i,t}]=x_{i,t}^{\top}\beta+\theta_{i}
\label{hypEq}
\end{equation}



Cette formulation correspond à un cas particulier du cas hybride proposé dans \cite{banditCtxtLinUCB}, en considérant une valeur de 1 pour la valeur du contexte propre à chaque action. Il est important de noter que plusieurs paramètres individuels auraient pu être considérés dans notre étude, cependant cette approche ne nous semble pas adaptée étant donné le nombre très élevé d'actions disponibles (qui mènerait à un apprentissage d'autant plus complexe). Ainsi, nous restreignons la modélisation individuelle à un terme unique de biais. L'utilisation d'un vecteur de paramètres commun permet une exploration facilitée, comme précédemment, grâce à la généralisation des corrélations observées pour des utilisateurs à l'ensemble des utilisateurs. Comme nous l'avons déjà vu, dans notre cas, une difficulté majeure provient du fait que tous les contextes ne sont pas observables, contrairement aux problèmes de bandits contextuels traditionnels. En effet les contraintes des différentes API ne nous autorisent pas à voir un contexte pour chaque action et on ne peut donc pas utiliser des algorithmes de bandits contextuels existants tels que \texttt{LinUCB} \cite{banditCtxtLinUCB} ou encore \texttt{OFUL} \cite{OFUL} par exemple. À l'instar du chapitre précédent, plusieurs cas sont envisageables concernant le processus choisissant les actions pour lesquelles un contexte est observable. On note par la suite $\mathcal{O}_{t} \subset \mathcal{K}$ l'ensemble des comptes pour lesquels un vecteur de contexte est disponible à l'itération $t$. Ainsi, le cas où $\mathcal{O}_{t}=\mathcal{K}$ correspond au bandit contextuel traditionnel. 


\begin{note}
Dans ce chapitre, les contextes sont par nature variables et sont directement observés par l'agent, contrairement au chapitre \ref{ModeleContextuelFixe} où seule une version bruitée était disponible.
\end{note}



Dans la section suivante, nous étudions dans un premier temps le cas le plus simple où tous les contextes sont observables. Ceci nous permettra de mettre en place les bases nécessaires à l'étude du cas plus complexe où une partie des contextes n'est pas accessible.


\section{Algorithmes}

Nous nous concentrons ici sur les algorithmes de types optimistes. Rappelons que le principe général, derrière toutes les politiques de ce type, consiste à construire  un intervalle de confiance sur les récompenses de chaque action. Pour ce faire, une des possibilités est de maintenir à jour des distributions a posteriori sur les différents paramètres du modèle. Certaines hypothèses doivent être faites à la fois sur la vraisemblance des observations, mais aussi sur les distributions a priori des paramètres. En particulier, l'utilisation des priors conjugués permet d'obtenir des solutions exactes. Dans notre étude, nous utiliserons des distributions gaussiennes.

\subsection{Intervalles de confiance lorsque les contextes sont visibles}


Construisons dans un premier temps un estimateur des paramètres dans le cas où tous les contextes seraient observables, avec les hypothèses suivantes :

\begin{itemize}
\item \textbf{Vraisemblance :} Les récompenses sont indépendamment  et identiquement distribuées selon les contextes observés: $r_{i,t} \sim \mathcal{N}(r_{i,t};x_{i,t}^{\top}\beta+\theta_{i},\sigma_{i}^2)$, avec $\sigma_{i}^2$ correspondant à la variance de l’écart entre la récompense $r_{i,t}$ et l'application linéaire de prédiction $x_{i,t}^{\top}\beta+\theta_{i}$; 
\item \textbf{Prior :} Les paramètres inconnus sont normalement distribués autour de l'origine: $\beta \sim \mathcal{N}(0,b^{2} \mathbb{I}_{d})$ et $\theta_{i} \sim \mathcal{N}(0,\rho_{i}^{2})$, où $b$ et $\rho_{i}$ permettent de contrôler la variance des paramètres et  $\mathbb{I}_{d}$ est la matrice identité de taille $d$ (taille des vecteurs de contexte). 
\end{itemize}


\begin{note}
L'hypothèse de vraisemblance gaussienne est plus restrictive que celle du chapitre \ref{ModeleContextuelFixe} dans lequel un bruit sous-gaussien était suffisant. 
\end{note}

Le but est de construire la distribution a posteriori des paramètres $\beta$ et $\theta_{i}$ à un instant $t$ connaissant les récompenses collectées, et les contextes associés, jusqu'à l'itération $t-1$. Pour alléger les notations, nous fixons $b$, $\rho_{i}$ et $\sigma_{i}$ à $1$ pour tout $i$. Cependant, tous les résultats peuvent être étendus à des cas plus complexes. 

Nous introduisons les notations matricielles condensées suivantes pour la suite du chapitre :

\begin{itemize}
\item $\mathcal{T}_{i,t-1}$ l'ensemble des itérations où $i$ a été choisi durant les $t-1$ premières étapes: $\mathcal{T}_{i,t-1}=\left\{s \leq t-1 , i \in \mathcal{K}_{s}\right\}$. On a donc $|\mathcal{T}_{i,t-1}|=N_{i,t-1}$;
\item $c_{i,t-1}$ le vecteur de récompenses obtenues par l'action $i$ lorsqu'elle a été choisie jusqu'au temps $t-1$: $c_{i,t-1}=(r_{i,s})_{s\in \mathcal{T}_{i,t-1}}$ ;
\item $D_{i,t-1}$ la matrice de taille $N_{i,t-1}\times d$ des contextes associée à $i$ lorsqu'elle a été choisie jusqu'au temps $t-1$: $D_{i,t-1}=(x_{i,s}^{\top})_{s\in \mathcal{T}_{i,t-1}}$.
\end{itemize}


Les deux propositions suivantes expriment les distributions a posteriori des paramètres du modèle à un instant $t$, avant que la sélection des actions n'ait été effectuée.


\begin{prop}
\label{propDistBetaChap3}
Les distributions a posteriori des paramètres $\beta$ et $\theta_{i}$ à l'étape $t$, lorsque tous les contextes sont visibles respectent:


\begin{equation}
\label{eqBetaChap3}
\beta \sim \mathcal{N}\left(\bar{\beta}_{t-1},V_{t-1}^{-1}\right)
\end{equation}

\begin{equation}
\label{eqThetaChap3}
\theta_{i}+\bar{x}_{i,t-1}^{\top}\beta  \sim \mathcal{N}\left(\bar{\mu}_{i,t-1},\frac{1}{N_{i,t-1}+1}\right)
\end{equation}


Où: 

\begin{align}
	 V_{t-1}=\mathbb{I}_{d}+\sum\limits_{i=1}^{K}  (N_{i,t-1}+1)\bar{\Sigma}_{i,t-1}& & b_{t-1}^{\top}=\sum\limits_{i=1}^{K}(N_{i,t-1}+1)\bar{\xi}_{i,t-1} & & \bar{\Sigma}_{i,t-1}=\dfrac{D_{i,t-1}^{\top}D_{i,t-1}}{N_{i,t-1}+1}-\bar{x}_{i,t-1}\bar{x}_{i,t-1}^{\top}\nonumber 
\end{align}
\begin{align}
  \bar{\xi}_{i,t-1}=\dfrac{c_{i,t-1}^{\top}D_{i,t-1}}{N_{i,t-1}+1}-\bar{\mu}_{i,t-1}\bar{x}_{i,t-1}^{\top} & & \bar{\beta}_{t-1}=V_{t-1}^{-1}b_{t-1}^{\top} & & \bar{\mu}_{i,t-1} = \dfrac{\sum\limits_{s\in \mathcal{T}_{i,t-1}} r_{i,s}}{N_{i,t-1}+1}  & & \bar{x}_{i,t-1} = \dfrac{\sum\limits_{s\in \mathcal{T}_{i,t-1}} x_{i,s}}{N_{i,t-1}+1} \nonumber
\end{align}



De plus, les variables aléatoires $\beta $ et $\bar{x}_{i,t-1}^{\top}\beta$  sont indépendantes.
\end{prop}

\begin{preuve}
Disponible en annexe \ref{PreuvePosteriorICWSM}.
\end{preuve}

\begin{note}
Tous ces paramètres peuvent être mis à jour de façon peu coûteuse à mesure que de nouveaux exemples d'apprentissage arrivent (la complexité de la mise à jour des paramètres est constante sur l'ensemble du processus). Nous détaillerons cette mise à jour plus tard lors de l'étude de l'algorithme.
\end{note}

On remarque que dans la proposition précédente, la distribution a posteriori des paramètres $\theta_{i}$ seuls n'est pas explicite. Le corollaire suivant permet d'obtenir cette distribution.

\begin{corol}
A l'étape $t$, la distribution des paramètres $\theta_{i}$ est telle que:

\begin{equation}
\label{eqThetaBisChap3}
\theta_{i} \sim \mathcal{N}\left(\bar{\mu}_{i,t-1}-\bar{x}_{i,t-1}^{\top}\beta_{t-1} ,\frac{1}{N_{i,t-1}+1} + \bar{x}_{i,t-1}^{\top}V_{t-1}^{-1}\bar{x}_{i,t-1}\right)
\end{equation}
\end{corol}

\begin{preuve}
En utilisant le fait que les variables aléatoires $\beta $ et $\bar{x}_{i,t-1}^{\top}\beta$  sont \textbf{indépendantes} et que $\theta_{i}=\theta_{i}+\bar{x}_{i,t-1}^{\top}\beta - \bar{x}_{i,t-1}^{\top}\beta =$\ref{eqThetaChap3}-$\bar{x}_{i,t-1}^{\top}$\ref{eqBetaChap3}, qui correspond à une combinaison linéaire de variables aléatoires indépendantes, on obtient le résultat souhaité.
\end{preuve}

\begin{prop}
 La valeur espérée $\mathbb{E}[r_{i,t}|x_{i,t}]$, de la récompense de l’utilisateur $i$ à l’itération $t$ sachant son contexte $x_{i,t}$, suit la distribution:
\begin{equation}
\label{distAllSeen}
\mathbb{E}[r_{i,t}|x_{i,t}] \sim 
\mathcal{N}\left(\bar{\mu}_{i,t-1}+(x_{i,t}-\bar{x}_{i,t-1})^{\top}\bar{\beta}_{t-1}, \frac{1}{N_{i,t-1}+1}+(x_{i,t}-\bar{x}_{i,t-1})^{\top}V_{t-1}^{-1}(x_{i,t}-\bar{x}_{i,t-1})\right)
\end{equation}
\end{prop}

\begin{preuve}
En remarquant que $\mathbb{E}[r_{i,t}|x_{i,t}]=x_{i,t}^{\top}\beta+\theta_{i}=(x_{i,t}-\bar{x}_{i,t-1})^{\top}\beta+\theta_{i}+\bar{x}_{i,t-1}^{\top}\beta$ et qu'il s'agit d'une combinaison linéaire des variables aléatoires \textbf{indépendantes} définies dans les équations \ref{eqThetaChap3} et \ref{eqBetaChap3}, on obtient le résultat souhaité.
\end{preuve}

\begin{theo}
\label{theoUCBICWSM}
Pour tout $0<\delta <1$ et $x_{i,t} \in \mathbb{R}^{d}$, en notant $\alpha = \Phi^{-1}(1-\delta/2)$ \footnote{$\Phi^{-1}$ est la fonction de répartition inverse d'une loi normale.}, pour chaque action $i$, après $t$ itérations:
\begin{multline}
P\Big( | \mathbb{E}[r_{i,t}|x_{i,t}] -  \bar{\mu}_{i,t-1}-(x_{i,t}-\bar{x}_{i,t-1})^{\top}\bar{\beta}_{t-1}| \ \leq \  \alpha \  \sigma_{i,t-1}  \Big)  \geq 1-\delta \\
\text{avec} \ \sigma_{i,t-1} = \sqrt{\dfrac{1}{N_{i,t-1}+1}+(x_{i,t}-\bar{x}_{i,t-1})^{\top}V_{t-1}^{-1}(x_{i,t}-\bar{x}_{i,t-1})}
\label{probObs}
\end{multline}
\end{theo}



\begin{preuve}
En utilisant l'équation \ref{distAllSeen}, on voit que la variable aléatoire $\dfrac{\mathbb{E}[r_{i,t}|x_{i,t}] -  \bar{\mu}_{i,t-1}-(x_{i,t}-\bar{x}_{i,t-1})^{\top}\bar{\beta}_{t-1}}{\sigma_{i,t-1}}$ suit une loi normale de moyenne 0 et de variance 1, d'où le résultat proposé.
\end{preuve}
 
 
Cette formule peut directement être utilisée pour définir une borne supérieure de l'intervalle de confiance (\textit{UCB - Upper Confidence Bound}) de la récompense espérée pour chaque utilisateur dont le contexte a été observé pour l’itération $t$:

\begin{equation}
s_{i,t} = \bar{\mu}_{i,t-1}+(x_{i,t}-\bar{x}_{i,t-1})^{\top}\bar{\beta}_{t-1} + \alpha\sqrt{\dfrac{1}{N_{i,t-1}+1}+(x_{i,t}-\bar{x}_{i,t-1})^{\top}V_{t-1}^{-1}(x_{i,t}-\bar{x}_{i,t-1})}
\label{obsScoreChap3}
\end{equation}
 
Ainsi les approches de type \textit{UCB} étant des approches optimistes, l'idée est alors de sélectionner à chaque instant $t$ les $k$ utilisateurs ayant les $k$ bornes $s_{i,t}$ les plus élevées. %  les utilisateurs avec les bornes supérieures les plus élevées. Dans notre cas, cela nous conduit à choisir à chaque instant $t$ les $k$ utilisateurs ayant le score $s_{a,t}$ le plus élevé, avec: 
Le score précédent pourrait directement être utilisé pour notre tâche de collecte d'information si tous les contextes de tous les utilisateurs étaient disponibles, ce qui n'est pas le cas, hormis lorsque $\mathcal{O}_{t}=\mathcal{K}$. Dans la section qui suit, nous étudions cette configuration spécifique qui nécessite un traitement particulier.



\subsection{Prise en compte des utilisateurs dont le contexte n'est pas visible} 


Les scores permettant de sélectionner les utilisateurs à écouter définis précédemment ne peuvent pas être calculés lorsque les contextes $x_{i,t}$ ne sont pas observés (c.-à-d. lorsque les utilisateurs ne sont pas dans $\mathcal{O}_{t}$). Cela nécessite donc une méthode permettant de qualifier les personnes dont le contexte est inconnu. De plus, cela implique des problématiques de mise à jour des paramètres appris lorsqu'un utilisateur a été écouté, mais dont le contexte n'a pas été révélé. 
Bien qu'il soit tentant de penser que le paramètre $\beta$ commun à tous et les paramètres individuels $\theta_{i}$ peuvent être appris séparément, ces derniers sont en réalité corrélés, comme le montrent les formules \ref{eqBetaChap3} et \ref{eqThetaChap3}. Il est important de remarquer que pour conserver les garanties probabilistes, les paramètres du problème ne devraient être mis à jour que lorsqu'un profil appartient à $\mathcal{K}_{t} \cap \mathcal{O}_{t}$. Si l'on remplace $\mathcal{T}_{i,t}$ par $\mathcal{T}_{i,t}^{both}=\left\{s \leq t , i \in \mathcal{K}_{t} \cap \mathcal{O}_{t} \right\}$ et $N_{i,t}$ par $N_{i,t}^{both}$, on peut alors réutiliser les formules de mise à jour des paramètres de la proposition \ref{propDistBetaChap3}. Ainsi le score de sélection de l'équation \ref{obsScoreChap3} est toujours valable.
Toutefois, pour un utilisateur dont le contexte est caché, cela n'est plus possible.


Pour pallier ce problème, nous proposons deux approches distinctes. La première, la plus intuitive consiste à effectuer un échantillonnage des contextes pour les utilisateurs dont ce dernier n'est pas visible. Cet échantillonnage sera effectué à partir d'une loi apprise sur chaque utilisateur. Dans la seconde approche, nous utiliserons la moyenne empirique des contextes lorsque ce dernier n'est pas directement observable. Nous verrons que cela fera intervenir un nouveau terme d'exploration visant à compenser l'incertitude induite par cette approximation.





\textbf{Notations supplémentaires:}
Nous introduisons les notations suivantes que nous utiliserons dans le reste du chapitre:

\begin{itemize}
\item L'ensemble des itérations où le contexte de $i$ a été observé au bout de $t$ étapes est noté $\mathcal{T}_{i,t-1}^{obs}=\left\{s \leq t-1 , i \in \mathcal{O}_{s} \right\}$ avec $|\mathcal{T}_{i,t-1}^{obs}| = n_{i,t-1}$. A nouveau à l'instant $t$, on utilisera les informations disponibles jusqu'au temps précédent, d'où la présence des indices $t-1$;
\item L'ensemble des observations du contexte de $i$ jusqu'à l'instant $t$ est noté $\mathcal{D}_{i,t-1}^{obs}=\left\{x_{i,s}\right\}_{s \in \mathcal{T}_{i,t-1}^{obs}}$;
\item La moyenne empirique des vecteurs de contexte de l’utilisateur $i$ à l'instant $t$ est notée $\hat{x}_{i,t-1}$, avec $\hat{x}_{i,t-1}=\dfrac{1}{n_{i,t-1}}\sum\limits_{s\in \mathcal{T}_{i,t-1}^{obs}} x_{i,s}$. Remarquons que $\hat{x}_{i,t-1}$ est différent de $\bar{x}_{i,t-1}$, car le premier est mis à jour à chaque fois que le contexte est observé tandis que le second l'est uniquement lorsque l'utilisateur a été observé et sélectionné lors d'une même itération.
\end{itemize}





\subsubsection{Modèle 1: échantillonnage des contextes}

\textbf{Idée générale: } Comme nous l'avons évoqué précédemment, l'idée est d'effectuer un apprentissage sur les utilisateurs afin d'être en mesure d'échantillonner leur contexte lorsque ce dernier n'est pas disponible. A l'instant $t$, lorsque l'on ne connaît pas $x_{i,t}$ pour un utilisateur $i$, il faudra effectuer un échantillonnage en se servant de  toutes les observations précédentes, c'est-à-dire $\mathcal{D}_{i,t-1}^{obs}$. A mesure que le contexte d'un utilisateur sera observé, le modèle sous-jacent sera de plus en plus fin et l'échantillonnage sera de plus en plus proche de la réalité. Pour ce faire, nous proposons d'utiliser un modèle probabiliste pour les distributions de contextes pour chaque compte $i$. On note $p(x_{i,t}|\gamma_{i})$ la distribution de contexte associée à un utilisateur $i$ paramétrée par $\gamma_{i}$. Selon les lois de probabilité utilisées $\gamma_{i}$ peut être un vecteur. Par exemple pour une loi normale en une dimension ce dernier représente la moyenne et la variance. Dans tous les cas, ce paramètre n'est pas connu par l'agent. Afin d'être en mesure de maintenir des distributions de probabilité sur les contextes en fonction des observations, on utilise également un modèle probabiliste pour les paramètres $\gamma_{i}$. On note $q(\gamma_{i})$ cette distribution. Finalement, en utilisant pour $q$ le prior conjugué de $p$ il est possible de maintenir une distribution a posteriori analytique sur les paramètres, notée $q(\gamma_{i}|\mathcal{D}_{i,t-1}^{obs})$ et sur les contextes, notée $p(x_{i,t}|\mathcal{D}_{i,t-1}^{obs})$. Dans la littérature cette dernière distribution est appelée la distribubution posterior prédictive. Toutes les distributions ne possèdent pas de prior conjugué, cependant c'est le cas pour la majorité des distributions usuelles. Selon les cas d'application, certaines distributions seront plus pertinentes que d'autres, comme nous le verrons dans la partie expérimentale \ref{XPChap3}. 


\textbf{Approximation du score de sélection: } En considérant les contextes $x_{i,t}$ de chaque action $i$ à chaque instant $t$ comme des variables aléatoires lorsque ces derniers ne sont pas disponibles, le score $s_{i,t}$ de l'équation  \label{obsScore} peut aussi être vu comme une variable aléatoire. En effet il s'agit d'une fonction de $x_{i,t}$ et d'autres valeurs fixées à un instant donné. Afin d'être en mesure d'attribuer un score aux actions dont le contexte n'est pas visible, nous proposons d'utiliser la valeur espérée de $s_{i,t}$ sachant les observations que nous avons effectuées dans le passé. Formellement, en notant $\tilde{s}_{i,t}$ ce nouveau score on a:


\begin{align*}
\forall i\notin \mathcal{O}_{t}: \tilde{s}_{i,t}&=\mathbb{E}[s_{i,t}|\mathcal{D}_{i,t-1}^{obs}]\\
&= \int_{x_{i,t}} s_{i,t}(x_{i,t} p(x_{i,t}|\mathcal{D}_{i,t-1}^{obs}) \, \mathrm dx_{i,t}
\end{align*}

Où nous avons explicitement fait apparaître la dépendance de $s_{i,t}$ en $x_{i,t}$ pour plus de clarté. On voit également apparaître $p(x_{i,t}|\mathcal{D}_{i,t-1}^{obs})$, la densité de probabilité apprise sur la distribution de contexte de l'action considérée. Malheureusement, l'expression ci-dessus n'est pas directement exploitable, car elle ne peut être calculée explicitement d'une façon générale et nécessite donc d'être approximée. On propose donc d'utiliser la méthode de Monte-Carlo suivante pour approximer l’intégrale :


\begin{align}
\label{scoreNotObsSampleChap3}
 \tilde{s}_{i,t} &\approx \dfrac{1}{L}\sum\limits_{x\in \mathcal{S}} s_{i,t}(x)\nonumber \\
 				&= \dfrac{1}{L}\sum\limits_{x\in \mathcal{S}} \bar{\mu}_{i,t-1}+(x-\bar{x}_{i,t-1})^{\top}\bar{\beta}_{t-1} + \alpha \ \sqrt{\dfrac{1}{N_{i,t-1}^{both}+1}+(x-\bar{x}_{i,t-1})^{\top}V_{t-1}^{-1}(x-\bar{x}_{i,t-1})}
\end{align}

Avec $\mathcal{S}=\left\{x \text{ échantilloné selon } p(x_{i,t}|\mathcal{D}_{i,t-1}^{obs})   \right\}$ un ensemble de $L$ échantillons provenant de la loi posterior prédictive $p(x_{i,t}|\mathcal{D}_{i,t-1}^{obs})$. Concrètement, ce score correspond à la moyenne empirique des scores calculés avec les échantillons présents dans $\mathcal{S}$. 



\textbf{Prise en compte de l'activité des utilisateurs :} Pour notre tâche en particulier, il s'avère que le contexte $x_{i,t}$ d'un utilisateur $i$ à un instant $t$ correspond au message qu'il a posté - à une transformation près - au temps $t-1$. Ainsi l'absence de message correspond à un contexte nul. Si l'on considère les itérations dans lesquelles le contexte d'un utilisateur $i$ a été vu avec le modèle précédent, il s'avère que les fois où ce dernier n'était pas actif seront tout de même considérées dans l'apprentissage de la loi $p(x_{i,t}|\mathcal{D}_{i,t-1}^{obs})$. D'un côté, ceci est positif puisque cela prend directement en compte l'activité des différents utilisateurs. En effet, les comptes peu actifs auront des distributions proches de 0. D'un autre côté, on perd en qualité la modélisation des messages postés en incorporant des exemples nuls de façon artificielle. Pour minimiser cet effet négatif tout en modélisant l'activité, nous allons dissocier l'activité d'un utilisateur et son contexte. D'une part, nous proposons de n'incorporer que les exemples où l'utilisateur a été actif, c'est-à-dire où $x_{i,t}\neq 0$, dans l'apprentissage de la loi $p(x_{i,t}|\mathcal{D}_{i,t-1}^{obs})$. D'autre part, nous introduisons une nouvelle variable aléatoire régissant la probabilité qu'a un utilisateur d'être actif à un instant $t$. Etant donné que l'on ne peut pas apprendre une probabilité pour chaque instant, nous subdivisons le processus de collecte en plusieurs périodes. Intuitivement, cela semble pertinent puisque dans le cadre des réseaux sociaux certains comptes seront forcément plus actifs selon le moment de la journée. Formellement, on définit une période comme un ensemble consécutif de $M$ itérations et l'on choisit un total de $nbPeriods$ périodes. A titre illustratif, si on considère qu'une itération dure une heure et que l'on choisit $nbPeriods=2$ et $M=12$, alors cela revient à diviser un jour complet en deux périodes dans lesquelles chaque utilisateur a une probabilité particulière d'être actif. Nous verrons dans la partie expérimentale différents choix possibles.

On associe à chaque utilisateur $i$ un vecteur $p_{i}\in \left[0..1\right]^{M}$ régissant sa probabilité d'être actif. On a donc $\mathbb{P}(i\text{ est actif au temps }t)=p_{i,j}$ lorsque $t$ est dans la période $j\in \left\{1,...,M \right\}$. Ainsi, la probabilité qu'un compte $i$ soit actif à un instant $t$ suit une loi de Bernoulli de probabilité $p_{i,j}$ lorsque $t$ est dans la période $j$. Ces probabilités n'étant pas connues a priori, elles doivent également être apprises à mesure que le temps avance. Pour ce faire, nous utilisons un prior sur chaque $p_{i,j}$ et on souhaite en déduire la distribution posterior prédictive $p_{i,j}$ sachant les observations passées, c'est-à-dire $\mathcal{D}_{i,t-1}^{obs}$. Le prior conjugué d'une loi de Bernoulli est une loi Beta de paramètre $a$ et $b$. Dans notre cas, aucune information n'étant disponible a priori, on choisit pour tous les comptes $a=b=1$, ce qui correspond à une loi uniforme. On introduit les deux notations qui nous seront utiles pour exprimer les probabilités qui nous intéressent :


\begin{itemize}
\item On note $S_{i,j,t-1}$ le nombre de fois où l'utilisateur $i$ a été \textbf{actif} lorsque son contexte a été observé jusqu'au temps $t$ dans la période $j$, c'est-à-dire: $S_{i,j,t-1}=|\left\{s \leq t-1 , i \in \mathcal{O}_{s},\text{$s$ est dans la période $j$}, x_{i,s}\neq 0 \right\}|$;
\item On note $F_{i,j,t-1}$ le nombre de fois où l'utilisateur $i$ a été \textbf{inactif} lorsque son contexte a été observé jusqu'au temps $t$ dans la période $j$, c'est-à-dire: $F_{i,j,t-1}=|\left\{s \leq t-1 , i \in \mathcal{O}_{s},\text{$s$ est dans la période $j$},x_{i,s}= 0 \right\}|$.
et $F_{i,j,t-1}$.
\end{itemize}



\begin{prop}
A l'instant $t$, la probabilité qu'a un utilisateur $i$ d'être actif suit une loi de Bernoulli telle que:


\begin{equation}
\mathbb{P}(i\text{ est actif au temps }t|\mathcal{D}_{i,t-1}^{obs})=\dfrac{S_{i,j,t-1}+1}{S_{i,j,t-1}+F_{i,j,t-1}+2}
\end{equation}
Où $j\in \left\{1,...,M \right\}$ correspond à la période dans laquelle se trouve $t$.
\end{prop}
 

\begin{preuve}
Etant donné une loi de Bernoulli de paramètre $p$ et en utilisant un prior Beta$(a,b)$ sur $p$, on montre en utilisant la règle de Bayes que le posterior sur $p$ au bout de $n$ observations est une loi Beta$(a+nbSucc,b+nbFail)$ où $nbSucc$ représente le nombre d'issues positif et $nbFail$ le nombre d'issues négatif parmi les $n$ observations. Par ailleurs, la distribution posterior prédictive et une loi de Bernoulli de paramètre $(a+nbSucc)/(a+nbSucc+b+nbFail)$. En utilisant les notations proposées plus haut on obtient directement le résultat annoncé.
\end{preuve}




Nous sommes maintenant en mesure de dériver un nouvel algorithme de bandit contextuel prenant en compte des contextes cachés, que nous appellerons \texttt{HiddenLinUCB-Sample} dans la suite. Nous le détaillerons à la fin de cette section dans l'algorithme \ref{HiddenLinUCB-Sample}. Ce dernier nécessite la définition d'un loi pour $p(x_{i,t}|\gamma_{i})$ et d'une d'un prior $q(\gamma_{i})$ pour chaque action. On supposera qu'il s'agit d'un prior conjugué de sorte qu'il est possible d'échantillonner selon la loi $p(x_{i,t}|\mathcal{D}_{i,t-1}^{obs})$ lorsque cela est nécessaire.
De plus dans cette version générique, on ne fait pas de supposition précise sur le processus délivrant les contextes c'est-à-dire sur la façon dont $\mathcal{O}_{t}$ est généré à chaque instant $t$. En revanche, pour faire partie de $\mathcal{K}$, une action doit être observée au moins une fois (au sens du contexte). Dans la partie expérimentale, nous proposerons diverses possibilités pour $\mathcal{O}_{t}$, à l'instar de ce qui a été fait dans le chapitre \ref{ModeleContextuelFixe}.
Finalement, afin d'alléger les notations, nous avons enlevé les dépendances en temps des différents paramètres. Cependant, le système de mise à jour de ces derniers respecte la logique du processus.


\begin{algorithm}[p]
\scriptsize
 \KwIn{$k$, $T$, $\alpha$, $L$, $M$}
 $V \leftarrow I_{d\times d}$ (matrice identité de taille $d$)\;
 $b \leftarrow 0_{d}$ (vecteur de 0 de dimension $d$)\;
 $\mathcal{K} \leftarrow \emptyset$\; 
\For{$t=1..T$} {
	$j$=période correspondant à l'itération $t$\;
	Recevoir $\mathcal{O}_{t}$\;	\label{getnewObservations}
	$\mathcal{K} = \mathcal{O}_{t} \cup \mathcal{K}$\; \label{feedArmSet}
    $\bar{\beta}=V^{-1}b$\;
    \For{$i  \in \mathcal{K}$} {
		\eIf {$i  \in \mathcal{O}_{t}$}{
        	\If {$i$ est nouveau}{
            	$N_{i}= 0$, $s_{i}= 0$, $\bar{\mu}_{i} =0$, $b_{i}= 0_{d}$, $\bar{x}_{i}=0_{d}$\;
				$\mathcal{D}_{i}^{obs}=\emptyset$, $p(x_{i}|\mathcal{D}_{i}^{obs})=q(\gamma_{i})$, $S_{i,k}=1$ pour tout $k\in \left\{1,...,M \right\}$, $F_{i,k}=1$ pour tout $k\in \left\{1,...,M \right\}$;\
            }
        Observer $x_{i,t}$\; \label{beginObserveAndUpdate}
        $\mathcal{D}_{i}^{obs}= \mathcal{D}_{i}^{obs} \cup \left\{x_{i,t}\right\}$\;
    	Mettre à jour  $p(x_{i}|\mathcal{D}_{i}^{obs})$ \;
        \eIf {$x_{i,t}$ est nul}{
        $F_{i,j}=F_{i,j}+1$
        }
        {
        $S_{i,j}=S_{i,j}+1$
        }
        \label{endObserveAndUpdate}
        
        $s_{i,t}=\bar{\mu}_{i}+(x_{i,t}-\bar{x}_{i})^{\top}\bar{\beta} + \alpha\sqrt{\dfrac{1}{N_{i}+1}+(x_{i,t}-\bar{x}_{i})^{\top}V^{-1}(x_{i,t}-\bar{x}_{i})}$ \;
        } 
        {
        \For{$j=1..L$} {
        	$s_{i,t}=0$\;
            $p_{i,t}=\dfrac{S_{i,j}+1}{S_{i,j}+F_{i,j}+2}$\;
        	Echantillonner  $isActive$ selon une loi de Bernouilli de paramètre $p_{i,t}$\;
            \eIf {$isActive=1$}{
            Echantillonner  $x$ selon $p(x_{i}|\mathcal{D}_{i}^{obs})$ \;
            $s_{i,t}=s_{i,t}+\left(\bar{\mu}_{i}+(x-\bar{x}_{i})^{\top}\bar{\beta} + \alpha\sqrt{\dfrac{1}{N_{i}+1}+(x-\bar{x}_{i})^{\top}V^{-1}(x-\bar{x}_{i})}\right)/L$\;
            }
            {
            $s_{i,t}=s_{i,t}+\left(\bar{\mu}_{i}-\bar{x}_{i}^{\top}\bar{\beta} + \alpha\sqrt{\dfrac{1}{N_{i}+1}+\bar{x}_{i}^{\top}V^{-1}\bar{x}_{i}}\right)/L$\;
            }
        	}
        }
		}
   	Sélectionner les $k$ actions ayant les scores les plus élevés:\\ 
    $\qquad\mathcal{K}_{t} \leftarrow \argmax\limits_{\hat{\mathcal{K}} \subseteq \mathcal{K}, |\hat{\mathcal{K}}|=k} \quad \sum\limits_{i \in \hat{\mathcal{K}}} s_{i,t}$ \; \label{userSelection}
    
    \For{$i  \in \mathcal{K}_{t}$} { \label{updateCountsBegin}
		Recevoir $r_{i,t}$\;
		\If{$i\in \mathcal{O}_{t}$}{
			$V= V+b_{i}b_{i}^{\top}/(N_{i}+1)$\;
			$b= b+b_{i}s_{i}/(N_{i}+1)$\;
			$N_{i}= N_{i}+1$\;
			$s_{i}= s_{i}+r_{i,t}$\;
            $\bar{\mu}_{i} = s_{i}/(N_{i}+1)$\;
			$b_{i}= b_{i}+x_{i,t}$\;
            $\bar{x}_{i}= b_{i}/(N_{i}+1)$\;
			$V= V+x_{i,t}x_{i,t}^{\top}-b_{i}b_{i}^{\top}/(N_{i}+1)$\;
			$V= b+r_{i,t}x_{i,t}-b_{i}s_{i}/(N_{i}+1)$
		}
	  } \label{updateCountsEnd}
	}
\caption{\texttt{HiddenLinUCB-Sample}}
\label{HiddenLinUCB-Sample}
\end{algorithm}


Dans la section suivante, nous proposons une autre approche basée sur l'estimation de la moyenne empirique du contexte de chaque action.

\subsubsection{Modèle 2: utilisation de la moyenne empirique}

\textbf{Hypothèses supplémentaires:} Afin de prendre en compte les contextes non visibles, nous effectuons les hypothèses suivantes:
\begin{itemize}
\item Sans perte de généralité, nous supposons que $\beta$ est borné par $S \in \mathbb{R}^{+*}$, c.-à-d. $||\beta|| \leq s $, où $||$ $||$ désigne la norme $l^{2}$ sur $\mathbb{R}^{d}$.
\item Pour tout $i$ et à chaque $t$, les contextes $x_{i,t} \in \mathbb{R}^{d}$  sont indépendants et identiquement distribués depuis une distribution inconnue de moyenne $x_{i}$ et variance $\Sigma_{i}$ finie. Dans la suite on suppose que l'on a $\Sigma_{i}=\gamma_{i}^{2}Id$ afin d'alléger les notations. A nouveau des cas plus complexes peuvent être pris en compte. 
\end{itemize}




\begin{note}
La dernière hypothèse n'est pas restrictive dans le sens où la forme des distributions n'est pas imposée par le modèle. L'hypothèse de variance finie - qui implique l'existence d'une espérance - est respectée pour la plupart des distributions usuelles.
\end{note}
 
 
\begin{theo}
\label{theoUCBICWSMBis}
Soit $0<\delta_1<1$ et $0<\delta_2<1$. En notant $M=\max\limits_{i\in\mathcal{K}}\gamma_{i}^{2}$ et $\mathbb{E}[r_{i,t}]$ l'espérance des récompenses de l'action $i$ prise sur les contexte, alors pour tout $t$ on a:
\begin{multline}
P\left(|\mathbb{E}[r_{i,t}] -\bar{\mu}_{i,t-1} - (\hat{x}_{i,t-1}-\bar{x}_{i,t-1})^{\top}\bar{\beta}_{t-1}| \leq  \alpha_{1} \ \hat{\sigma}_{i,t-1} +   \alpha_{2}\sqrt{\dfrac{1}{n_{i,t-1}}} \right) \geq  
1-\delta_{1}-\delta_{2} \\
\text{avec} \ \hat{\sigma}_{i,t-1} = \sqrt{\dfrac{1}{N_{i,t-1}^{both}+1} + (\hat{x}_{i,t-1}-\bar{x}_{i,t-1})^{\top}V_{t-1}^{-1}(\hat{x}_{i,t-1}-\bar{x}_{i,t-1})} 
\label{probNonObs}
\end{multline}
 où $\alpha_{1}=\Phi^{-1}(1-\delta_{1}/2)$ et $\alpha_{2}=S\sqrt{\dfrac{Md}{\delta_{2}}}$
\end{theo}

\begin{preuve}
La preuve complète est disponible en annexe \ref{PreuveUCBICWSMBis}.
\end{preuve}


Ainsi, l'inégalité ci-dessus nous donne une borne relativement serrée de l'intervalle de confiance associé à la récompense espérée de l’utilisateur $i$, d'où nous pouvons dériver un nouveau score de sélection. À chaque itération $t$, si le contexte de $i$ n'est pas observé, son score noté $\tilde{s}_{i,t}$ est tel que:

\begin{equation}
\tilde{s}_{i,t}=\bar{\mu}_{i,t-1}+(\hat{x}_{i,t-1}-\bar{x}_{i,t-1})^{\top}\bar{\beta}_{t-1} + \alpha_{1} \sqrt{\dfrac{1}{N_{i,t}^{both}+1} + (\hat{x}_{i,t}-\bar{x}_{i,t})^{\top}V_{t}^{-1}(\hat{x}_{i,t}-\bar{x}_{i,t})} +  \alpha_{2}\sqrt{\dfrac{1}{n_{i,t-1}}}
\label{scoreNotObsMeanChap3}
\end{equation}


Notons que le terme d'exploration supplémentaire $\sqrt{\dfrac{1}{n_{i,t-1}}}$ tend vers 0 à mesure que le nombre d’observations de $i$ augmente, et le score tend donc vers un score \texttt{LinUCB} \cite{banditCtxtLinUCB} classique (comme dans l'équation \ref{obsScoreChap3}) dans lequel le contexte est remplacé par sa moyenne empirique $\hat{x}_{i,t-1}$. Notons que si la probabilité qu'un contexte soit visible et $0<p<1$ on peut affirmer que $\sqrt{\dfrac{1}{n_{i,t-1}}}$ tend bien vers 0 lorsque $t$ est suffisamment grand.

\begin{note}
Si l'on souhaite avoir une probabilité égale pour les cas (contexte observé et non observé), il suffira de prendre $\delta_{1}=\delta_{2}=\delta/2$.
\end{note}

A nouveau, nous sommes en mesure de dériver un nouvel algorithme de bandit contextuel avec contextes cachés. Nous appellerons ce dernier \texttt{HiddenLinUCB-Mean} dans la suite. Ce dernier est détaillé ci-après dans l'algorithme \ref{HiddenLinUCB-Mean}. Comme précédemment, nous avons enlevé les dépendances en temps des différents paramètres.


\begin{algorithm}[p]
\scriptsize
 \KwIn{$k$, $T$, $\alpha$,$\alpha_1$,$\alpha_2$}
 $V \leftarrow I_{d\times d}$ (matrice identité de taille $d$)\;
 $b \leftarrow 0_{d}$ (vecteur de 0 de dimension $d$)\;
 $\mathcal{K} \leftarrow \emptyset$\; 
 $\bar{\beta}=V^{-1}b$\;
\For{$t=1..T$} {
	Recevoir $\mathcal{O}_{t}$\;	\label{getnewObservationsBis}
	$\mathcal{K} = \mathcal{O}_{t} \cup \mathcal{K}$\; \label{feedArmSetBis}
    \For{$i  \in \mathcal{K}$} {
		\eIf {$i  \in \mathcal{O}_{t}$}{
        	\If {$i$ est nouveau}{
            	$N_{i}= 0$, $s_{i}= 0$, $\bar{\mu}_{i} =0$, $b_{i}= 0_{d}$, $\bar{x}_{i}=0_{d}$\;
                $n_{i}=0$, $\hat{x}_{i}=0_{d}$\; 
            }
        Observer $x_{i,t}$\; \label{beginObserveAndUpdateBis}
        $\hat{x}_{i}=(n_{i}\hat{x}_{i}+x_{i,t})/(n_{i}+1)$\;
        $n_{i}=n_{i}+1$  \; \label{endObserveAndUpdateBis}
        
        $s_{i,t}=\bar{\mu}_{i}+(x_{i,t}-\bar{x}_{i})^{\top}\bar{\beta} + \alpha\sqrt{\dfrac{1}{N_{i}+1}+(x_{i,t}-\bar{x}_{i})^{\top}V^{-1}(x_{i,t}-\bar{x}_{i})}$ \;
        } 
        {
        $s_{i,t}=\bar{\mu}_{i}+(\hat{x}_{i}-\bar{x}_{i})^{\top}\bar{\beta} +\alpha_{1}\sqrt{\dfrac{1}{N_{i}+1}+(\hat{x}_{i}-\bar{x}_{i})^{\top}V^{-1}(\hat{x}_{i}-\bar{x}_{i})} +  \alpha_{2}\sqrt{\dfrac{1}{n_{i}}}$\;
        }
		}
   	Sélectionner les $k$ actions ayant les scores les plus élevés:\\ 
    $\qquad\mathcal{K}_{t} \leftarrow \argmax\limits_{\hat{\mathcal{K}} \subseteq \mathcal{K}, |\hat{\mathcal{K}}|=k} \quad \sum\limits_{i \in \hat{\mathcal{K}}} s_{i,t}$ \; \label{userSelectionBis}
    
    \For{$i  \in \mathcal{K}_{t}$} { \label{updateCountsBeginBis}
		Recevoir $r_{i,t}$\;
		\If{$i\in \mathcal{O}_{t}$}{
			$V= V+b_{i}b_{i}^{\top}/(N_{i}+1)$\;
			$b= b+b_{i}s_{i}/(N_{i}+1)$\;
			$N_{i}= N_{i}+1$\;
			$s_{i}= s_{i}+r_{i,t}$\;
            $\bar{\mu}_{i} = s_{i}/(N_{i}+1)$\;
			$b_{i}= b_{i}+x_{i,t}$\;
            $\bar{x}_{i}= b_{i}/(N_{i}+1)$\;
			$V= V+x_{i,t}x_{i,t}^{\top}-b_{i}b_{i}^{\top}/(N_{i}+1)$\;
			$V= b+r_{i,t}x_{i,t}-b_{i}s_{i}/(N_{i}+1)$
		}
	  } \label{updateCountsEndBis}
	}
\caption{\texttt{HiddenLinUCB-Mean}}
\label{HiddenLinUCB-Mean}
\end{algorithm}


\subsubsection{Un mot sur le regret}

Bien que l'algorithme \texttt{LinUCB} classique soit extrêmement performant et rapide d'un point de vue expérimental \cite{banditCtxtLinUCB}, son analyse théorique pose des difficultés techniques. En effet, comme le font remarquer les auteurs dans \cite{banditCtxtLinUCBpreuve}, pour pouvoir utiliser l'inégalité de Azuma-Hoeffding, il faut que les estimateurs de récompenses à chaque itération proviennent d'une combinaison linéaire de récompenses passées indépendantes. Or l'algorithme \texttt{LinUCB} calcule un estimateur de $\beta$ qui dépend des choix précédents. Pour outrepasser cette difficulté, les auteurs modifient ce dernier en \texttt{BaseLinUCB}, qui est basé sur des échantillons indépendants, et surplombé d’un algorithme nommé \texttt{SupLinUCB} qui permet de s'assurer que cette hypothèse est vérifiée en pratique. Notons que l’algorithme \texttt{OFUL}, permettant également de résoudre le problème du bandit contextuel, peut être étudié directement grâce au processus auto normalisé (voir chapitre précédent). 

Ainsi, l'étude du regret des deux algorithmes proposés nécessiterait d'une part les outils utilisés dans \cite{banditCtxtLinUCBpreuve}, mais aussi la quantification de l'impact de l'approximation effectuée en utilisant soit des échantillons (comme dans \texttt{HiddenLinUCB-Sample}) soit la moyenne empirique (comme dans \texttt{HiddenLinUCB-Mean}) à la place de la véritable valeur du contexte. En effet bien que les estimateurs soient de plus en plus précis à mesure que le nombre d'observations augmente, l'erreur potentiellement faite, sommée sur tous les pas de temps peut dans certains cas ne pas être sous-linéaire. Pour illustrer ce propos, prenons un cas très simple avec $K=2$, $k=1$, $d=1$, $\beta=1$, $\theta_{1}=\theta_{2}=0$. 
Dans ce cas, d'après la définition \ref{defPseudoRegCtxt}, le pseudo-regret cumulé vaut: $\hat{R}_{T}=\sum\limits_{t=1}^{T} x_{i^{\star}_{t},t}-x_{i_{t},t}$,
 où à l'instant $t$ on a $i^{\star}_{t}=\argmax\limits_{i=1,2} x_{i,t}$. 
En l'absence de supposition sur les distributions de $x_{1,t}$ et $x_{2,t}$, il est clair que l'algorithme \texttt{HiddenLinUCB-Sample} ne peut être appliqué. En revanche, l'algorithme \texttt{HiddenLinUCB-Mean} ne se servant que de la moyenne empirique est utilisable. Supposons que le processus de génération de $\mathcal{O}_{t}$ est le suivant : pendant les $T_{0}<T$ premiers pas de temps $\mathcal{O}_{t}=\mathcal{K}$ et pendant les $T-T_{0}$ derniers pas de temps $\mathcal{O}_{t}=\emptyset$. 
On suppose de plus que $x_{i,t}$ vaut 1 pour le bras optimal et 0 pour l'autre, c'est à dire $x_{i,t}=\mathbb{1}_{\left\{i=i^{\star}_{t}\right\}}$. Supposons de plus que le bras optimal est généré de façon aléatoire, uniformément à chaque étape. Ainsi, les hypothèses de moyennes et variances finies sont bien respectées. Cependant, dans ce cas l'estimateur $\hat{x}_{i,t}$, utilisé dans le score de sélection dès lors que $t>T_{0}$ sera le même en moyenne pour tous les bras et donc notre politique \texttt{HiddenLinUCB-Mean} ne serait pas en mesure de distinguer l'action optimale. En effet, en considérant des termes de biais nuls dans le modèle, dans ce cas précis, le score de sélection de l'algorithme s'écrit: 
$s_{i,t}=\hat{x}_{i,t-1}^{\top}\bar{\beta}_{t-1}+\alpha_{1} \sqrt{ \hat{x}_{i,t}^{\top}V_{t}^{-1}\hat{x}_{i,t}}$. Finalement, il apparaît que le regret, qui peut s'écrire $\hat{R}_{T}=\sum\limits_{t=1}^{T} \mathbb{1}_{\left\{i_{t}\neq i^{\star}_{t}\right\}}$ grandira de façon linéaire. Nous venons donc d'extraire une situation dans laquelle les hypothèses énumérées plus haut sont respectées et où notre algorithme ne peut atteindre un regret sous-linéaire.





\subsubsection{Conclusion}

Dans le cadre de notre tâche de collecte d'information en temps réel, nous avons dans cette partie étudié un nouveau problème de bandit contextuel dans lequel à chaque itération, le contexte d'un certain nombre d'actions n'est pas accessible. Nous avons proposé deux méthodes distinctes permettant de prendre en compte les actions dont le profil est caché dans le processus de sélection à chaque itération. La première se base sur un échantillonnage des contextes manquants dans lequel on modélise directement la probabilité d'un utilisateur d'être actif à un certain instant, tandis que la seconde utilise un estimateur de leur moyenne comme approximation. Dans la partie suivante, nous proposons d'effectuer des expérimentations sur des données artificielles et sur des données de médias sociaux.





\section{Expérimentations}

\label{XPChap3}

	\subsection{Données artificielles}
    
    \subsubsection{Protocole}
        
         \textbf{Génération des données:} Afin d'évaluer les performances de notre algorithme nous l'expérimentation dans un premier temps sur des données simulées. Pour cela, on fixe un horizon de $T=5000$ pas de temps, un ensemble de $K=500$ actions et $d=10$ dimensions. On fixe le nombre de périodes à $M=8$ et le nombre de pas de temps par période à $nbStepsPerPeriod=10$. On tire ensuite un vecteur de régression $\beta$ aléatoirement dans $\left[-S/\sqrt{d}..S/\sqrt{d}\right]^{d}$, de façon à respecter la condition $||\beta||\leq S =1$. Pour chaque bras $i$ on tire un vecteur aléatoire $x_{i}$ depuis une loi normale $\mathcal{N}(0,Id)$ de dimension $d$ et un paramètre $\theta_{i}$ depuis une loi normale $\mathcal{N}(0,1)$. Pour finir, on tire uniformément dans $\left[0..1\right]^{M}$ un vecteur $p_{i}$ pour chaque action $i$. Ensuite, pour chaque itération $t \in \left\{1,...,T \right\}$ du processus, on procède de la façon suivante pour simuler les données:
    
    \begin{enumerate}
    	\item On calcule $j$, la période dans laquelle se trouve $t$;
    	\item Pour chaque $i \in \left\{1,...,K \right\}$
        	\begin{enumerate}
        		\item on tire un variable $isActive$ selon une loi de Bernoulli de paramètre $p_{i,j}$;
                \item \textbf{si} $isActive$ est vraie alors n tire un échantillon $x_{i,t}$ suivant une loi uniforme normale $\mathcal{N}(x_{i},Id)$;
                \item \textbf{sinon} $x_{i,t}=0$.
        	\end{enumerate}
        \item Pour chaque $i \in \left\{1,...,K \right\}$, on tire une récompense $r_{i,t}$ selon une normale $\mathcal{N}(x_{i,t}^{\top}\beta+\theta_{i},1)$;
        \item Pour chacune des politiques étudiées, on sélectionne un ensemble $\mathcal{K}_{t}$ de $k=10$ actions pour lesquelles on récolte la récompense correspondante.
    \end{enumerate}

Ce processus est répété 1000 fois puis moyenné.
    

   
	\textbf{Politiques testées:} Les algorithmes de bandits contextuels existants ne semblent pas bien adaptés pour traiter notre problème de bandit avec contextes cachés. En effet, ces derniers ne peuvent pas prendre les actions dont le contexte n'est pas disponible à un instant donné dans le processus de sélection. Contrairement au cas du chapitre précédent, ici, notre problème ne peut pas se voir directement comme un problème de bandit stationnaire. Cependant, en prenant l'espérance des récompenses de chaque action $i$ selon les profils, nous avons montré que l'on a $\mathbb{E}[r_{i,t}]=x_{i}^{\top}\beta + \theta_{i}$. Ainsi les algorithmes de bandits stationnaires peuvent être en mesure de détecter cette valeur de biais. Cependant, ces derniers ne peuvent pas exploiter les valeurs réelles des contextes observés.
  Nous choisissons de nous comparer aux algorithmes suivants : \texttt{CUCB}, \texttt{CUCBV}, \texttt{MOSS} et un algorithme \texttt{Thompson Sampling} avec récompense gaussienne décrite dans l'état de l'art, et initialement proposé par \cite{banditSimpleThompsonAnalysis2}. Soulignons que ces trois politiques n'utilisent aucune information extérieure autre que les récompenses observées. 
  D'autre part, nous implémentons les deux politiques que nous avons proposées, à savoir  \texttt{HiddenLinUCB-Sample} et \texttt{HiddenLinUCB-Mean} respectivement décrits dans les algorithmes \ref{HiddenLinUCB-Sample} et \ref{HiddenLinUCB-Mean}. Pour \texttt{HiddenLinUCB-Sample} nous fixons le nombre d'échantillons à une valeur de $L=50$ et le nombre de périodes à $M=8$. On fixe de plus $\delta=0.05$, ce qui correspond à une valeur de $\alpha=1.96$. Pour \texttt{HiddenLinUCB-Mean}, on utilise également $\alpha=\alpha_{1}=\alpha_{2}=1.96$. Finalement, pour chacune de ces deux politiques, nous implémentons les trois scénarios présentés au chapitre précédent pour le processus générant l'ensemble $\mathcal{O}_{t}$ à chaque itération. On rappelle que dans le cas 1 on a $\mathcal{O}_{t}=\mathcal{K}$, dans le cas 2, chaque action a une probabilité $p$ d'être dans $\mathcal{O}_{t}$ à chaque pas de temps et dans le cas 3, $\mathcal{O}_{t}=\mathcal{K}_{t-1}$. Ainsi, dans le cas 3, chaque action doit être sélectionnée au moins une fois afin de lui permettre d'entrer dans l'ensemble $\mathcal{K}$. On forcera donc l'algorithme à agir de la sorte. On compare différentes valeurs de $p\in \left\{0,0.1,0.2, 0.5,0.7, 1 \right\}$ où l'on rappelle que par convention $p=0$ correspondant au cas 3 et $p=1$ au cas 1. Lorsque $p=1$, les deux algorithmes sont identiques et on les notera \texttt{LinUCB}, ce qui correspond à la version traditionnelle.
	
    \textbf{Echantillonnage des contextes non disponibles: } L'algorithme \texttt{HiddenLinUCB-Sample} effectue à chaque itération, et pour les actions dont le profil n'est pas visible, un certain nombre d'échantillonnages. En effet d'une part une variable aléatoire décide si oui ou non un contexte est émis, puis, dans le cas positif, le contexte lui-même doit être échantillonné selon la loi posterior prédictive $p(x_{i}|\mathcal{D}_{i,t-1}^{obs})$. Afin d'être en mesure de maintenir une distribution analytique et échantillonnable, il est nécessaire de faire des hypothèses, selon les cas d'usages, sur les contextes. Dans ce cas, conformément à la loi utilisée pour la génération des données, on fait l'hypothèse que les contextes $x_{i,t}$ sont gaussiens, de variance $\Sigma =Id$ et de moyenne $\mu_{i}$. Afin de rester dans un cadre probabiliste on place un prior, également gaussien sur chaque $\mu_{i}$ de moyenne nulle et de variance $\Sigma_{0} =Id$. Ainsi, l'application du théorème Bayes permet d'affirmer que la distribution a posteriori des $\mu_{i}$ est telle que\footnote{Il s'agit d'un résultat classique en inférence bayésienne}:

    
    \begin{equation*}
    p(\mu_{i}|\mathcal{D}_{i,t-1}^{obs}) \sim \mathcal{N}\left(\mu_{i};(\Sigma_{0}^{-1} + n_{i,t-1}\Sigma^{-1})n_{i,t-1}\Sigma^{-1}\hat{x}_{i,t-1}, (\Sigma_{0}^{-1} + n_{i,t-1}\Sigma^{-1})^{-1}\right)
    \end{equation*}

D'où l'on obtient la distribution posterior prédictive qui nous intéresse pour effectuer l’échantillonnage :


    \begin{equation*}
    p(x_{i,t}|\mathcal{D}_{i,t-1}^{obs}) \sim \mathcal{N}\left(x_{i,t};(\Sigma_{0}^{-1} + n_{i,t-1}\Sigma^{-1})n_{i,t-1}\Sigma^{-1}\hat{x}_{i,t-1}, (\Sigma_{0}^{-1} + n_{i,t-1}\Sigma^{-1})^{-1}+\Sigma\right)
    \end{equation*}

On remarque qu'à un instant $t$ cette distribution ne dépend que des itérations précédentes. Dans les expérimentations sur données réelles on utilisera une autre hypothèse sur les distributions de contextes, plus réaliste, ce qui nous conduira à une tout autre forme de loi posterior prédictive.



 	\subsubsection{Résultats}
    
    Nous proposons de mesurer les performances de nos algorithmes en termes de regret cumulé $R_{t}$ dont nous rappelons la définition:
    \begin{equation*}
\sum\limits_{s=1}^{t} \sum\limits_{i\in \mathcal{K}_{s}^{\star}} r_{i,s} - \sum\limits_{i\in \mathcal{K}_{s}} r_{i,s}
    \end{equation*}  
    où $\mathcal{K}_{s}^{\star}$ est  l'ensemble des $k$ actions ayant la plus grande valeur de $x_{i,s}^{\top}\beta+\theta_{i}$. La figure \ref{fig:regretVsTimeSimHiddenLinUCB} représente l'évolution du regret cumulé au cours du temps pour les différents algorithmes testés. Afin d'améliorer la lisibilité, on ne représente que  les cas $p=0.5$, $p=0.1$ et $p=0.0$ pour les algorithmes \texttt{HiddenLinUCB-Sample} et \texttt{HiddenLinUCB-Mean}. Nous ferons une analyse des autres cas ultérieurement. La première chose à noter est que la politique \texttt{Random} offre de moins bonnes performances que tous les algorithmes de bandit stationnaires, à savoir \texttt{CUCB}, \texttt{CUCBV}, \texttt{MOSS} et \texttt{Thompson Sampling}. Ceci confirme que ces derniers sont en mesure d'apprendre les composantes de biais sur les différents bras. On remarque que les trois politiques \texttt{CUCB}, \texttt{MOSS} et \texttt{Thompson Sampling} offrent des performances quasi égales tandis que \texttt{CUCBV} est légèrement moins bon. La variance de toutes les actions étant la même ce dernier ne peut pas en tirer parti. Plus intéressant est le fait que dans toutes les configurations (c.-à-d. pour n'importe quelle valeur de $p$) les algorithmes \texttt{HiddenLinUCB-Sample} et \texttt{HiddenLinUCB-Mean} offrent de meilleurs résultats que les politiques de bandits stationnaires, toutes confondues. On note d'une façon générale que pour un algorithme donné (\texttt{HiddenLinUCB-Sample} ou \texttt{HiddenLinUCB-Mean}) les performances se dégradent à mesure que $p$ diminue, et a fortiori sont maximums pour $p=1$, c'est-à-dire pour la politique \texttt{LinUCB}. Ceci semble cohérent, étant donné que plus $p$ est grand, plus la qualité des estimateurs est élevée et le nombre de fois où l'on a à s'en servir est faible. En revanche lorsque $p$ est petit, on dispose de moins d'exemples pour maintenir les estimateurs de contexte, et l'on doit souvent s'en servir pour calculer les scores de sélection des actions dont le contexte n'est pas disponible à un instant donné. On remarque finalement que pour une valeur de $p$ fixée, l'algorithme \texttt{HiddenLinUCB-Sample} est toujours meilleur que l'algorithme \texttt{HiddenLinUCB-Mean}. De plus, cet effet est accentué lorsque les valeurs de $p$ diminuent. Le paragraphe ci-dessous fait une étude plus précise de ce comportement.



               \begin{figureth}
			\includegraphics[width=0.7\linewidth]{HiddenLinUCBSimulationK500T5000Regret.pdf}
        \caption[Regret simulation \texttt{HiddenLinUCB}]{Regret cumulé en fonction du temps pour l'expérience sur données artificielles.}
			\label{fig:regretVsTimeSimHiddenLinUCB}
			\end{figureth}
 
 
La figure \ref{fig:regretFinalBowplotHiddenLinUCB} représente le diagramme en boîte de la valeur finale du regret sur les 1000 tests effectués pour les algorithmes \texttt{HiddenLinUCB-Mean} et \texttt{HiddenLinUCB-Sample} pour toutes les valeurs de $p$ proposées. L'idée selon laquelle pour une probabilité donnée, l'algorithme \texttt{HiddenLinUCB-Sample} offre de meilleures performances que \texttt{HiddenLinUCB-Mean} se confirme bien ici. De plus cet effet s'estompe bien lorsque $p$ augmente. Ce résultat est principalement dû au fait que nous avons généré des données selon un modèle prenant l'inactivité des certaines actions (au sens contexte nul) selon les périodes, et que l'algorithme \texttt{HiddenLinUCB-Sample} parvient donc à mieux modéliser l’environnement que son concurrent. Cependant, il est beaucoup plus coûteux, car il nécessite à la fois plus de mémoire, mais aussi des temps de calcul plus importants du fait qu'il doive échantillonner un grand nombre de variables aléatoires. Nous remarquons aussi que la variabilité des résultats est d'autant plus grande que $p$ diminue. Ceci peut s'expliquer d'un côté par le fait que le processus générant $\mathcal{O}_{t}$ est plus variable, mais également par le fait que les estimateurs utilisés sont moins précis (et donc plus variables). D'ailleurs, l'algorithme \texttt{HiddenLinUCB-Sample}, qui possède lui-même une source d'incertitude due à l'échantillonnage a globalement plus de variabilité.  %Finalement, notons que l'algorithme \texttt{HiddenLinUCB-Sample} pour le cas $p=0$ est plus performant que l'algorithme \texttt{HiddenLinUCB-Mean} pour $p=0.1$. 

              \begin{figureth}
			\includegraphics[width=0.7\linewidth]{HiddenLinUCBSimulationK500T5000BoxplotFinalRegret.pdf}
        \caption[Diagramme en boîte du regret final \texttt{HiddenLinUCB}]{Diagramme en boîte du regret final obtenu avec les algorithmes \texttt{HiddenLinUCB-Mean} et \texttt{HiddenLinUCB-Sample} pour différentes valeurs de $p\in \left\{0,0.1,0.2, 0.5,0.7, 1 \right\}$.}
			\label{fig:regretFinalBowplotHiddenLinUCB}
			\end{figureth}
            
            Dans la section qui suit, nous expérimentons nos algorithmes sur des données réelles.

	\subsection{Données réelles}

Nous venons de voir que les algorithmes proposés dans le chapitre offrent de bonnes performances sur des données simulées respectant bien les hypothèses. Nous proposons maintenant d'expérimenter ces mêmes algorithmes dans le cadre de notre tâche de collecte d'information sur Twitter. Nous nous évaluerons à la fois sur des jeux de données, mais aussi dans une expérimentation en conditions réelles.


		\subsubsection{Hors ligne}


		\paragraph{Modèle de contexte}
        
        
On se place dans le même cadre que dans le chapitre précédent (c.f. \ref{modelProfilStat}) dans lequel, à un instant $t$, nous utilisions les messages postés au temps $t-1$ comme échantillons de profils à l'instant $t$ (pour les utilisateurs appartenant à $\mathcal{O}_{t}$. Formellement nous avions $x_{i,t}=F(\omega_{i,t-1})$ où $\omega_{i,t-1}$ représente les messages du compte $i$ à l'instant $t-1$ et $F$ est une transformation nous permettant de réduire la dimension de l'espace des profils. Nous proposons d'utiliser cette même représentation pour modéliser le contexte d'un utilisateur à un instant donné. Cependant, ces derniers ne seront pas utilisés de la même façon que dans le chapitre précédent dans l'algorithme de collecte de données. On remarquera que ce modèle a l'avantage de modéliser indirectement l'activité des utilisateurs. En effet, un contexte nul est équivalent à une absence d'activité d'un utilisateur sur le réseau social à un instant donné. En revanche, il est évidemment possible qu'un compte publie à un instant $t$ sans pour autant avoir été actif au temps $t-1$, d'où la présence du terme de biais dans notre modèle. Nous pouvons désormais appliquer l'algorithme \texttt{HiddenLinUCB-Mean} directement, par contre l'algorithme \texttt{HiddenLinUCB-Sample} nécessite quant à lui un modèle probabiliste de la distribution des contextes pour qu'il soit en mesure de les échantillonner lorsque ces derniers ne sont pas disponibles (c.-à-d. pour tous les utilisateurs n'étant pas dans $\mathcal{O}_{t}$ à un instant $t$). Comme nous l'avons déjà précisé dans le chapitre précédent, la fonction $F$ appliquée au message correspond dans notre cas à une transformation LDA. En regardant de plus près ce modèle, il apparaît que les composantes du vecteur de sortie suivent une loi de Dirichlet. Ainsi, un choix judicieux pour modéliser les contextes de façon probabiliste serait d'utiliser une loi de Dirichlet. Or cette dernière ne possède pas de prior conjugué, rendant ainsi complexe un apprentissage des lois a posteriori. Afin s'affranchir de cette difficulté tout en restant réalistes, nous choisissons de modéliser directement les messages publiés par les utilisateurs. Dans cette optique, on utilise un modèle sac de mot pour la représentation des messages. Etant donné un dictionnaire de taille $m$, un message $\omega_{i,t-1}$ est représenté comme un vecteur de $\mathbb{N}^{m}$, où la composante $k$ est égale au nombre d'occurrences du mot $k$ dans le message. Afin de rester dans un cadre probabiliste, on fait l'hypothèse que ces derniers proviennent de lois multinomiales à $m$ issues, où le nombre de tirages correspond au nombre de mots dans un message. Pour restreindre la taille des vecteurs de probabilités, nous limitons le nombre de mots du dictionnaire. Dans cette optique, nous avons appliqué un \textit{Stemmer} à l'ensemble des messages des bases de données puis nous avons calculé les scores TF-IDF de chaque terme. Nous ne conservons que les $m=2000$ mots les plus importants dans notre dictionnaire final. Pour chaque compte $i$, on note $p_{i}$ le vecteur de probabilité de chaque mot. Le prior conjugué de la loi multinomiale est la distribution de Dirichlet de dimension $m$. Cette dernière possède un paramètre noté $a=a_{1},..,a_{m}$. Ainsi la distribution a posteriori de $p_{i}$ étant donné les observations $\mathcal{D}_{i,t-1}^{obs}$ est une loi de Dirichlet telle que:

    \begin{equation*}
    p(p_{i}|\mathcal{D}_{i,t-1}^{obs}) = Dir(a+\sum\limits_{s\in \mathcal{T}^{obs}_{i,t-1}}\omega_{i,s})
    \end{equation*}

Par ailleurs, la distribution posterior prédictive est une loi de Dirichlet-Multinomiale de paramètre $a^{post}=a+\sum\limits_{s\in \mathcal{T}^{obs}_{i,t-1}}\omega_{i,s}$. L'échantillonnage d'un message selon cette loi s'effectue de la façon suivante : premièrement, on fait un tirage de $m$ valeurs selon $m$ distributions Gamma de paramètre $a^{'}_{k}$ pour $k\in \left\{1,m\right\}$. On normalise ensuite chaque valeur par la somme de toutes les composantes pour avoir un vecteur de probabilités. On effectue ensuite $l$ tirages selon cette probabilité, ou $l$ est la taille du message que l'on souhaite générer. Nous avons fixé à $l=50$ mots pour tous les utilisateurs. Notons qu'il serait également possible d'effectuer un apprentissage sur la taille des messages de chaque utilisateur. Finalement, une fois un message échantillonné, la fonction $F$ lui est appliquée pour créer un contexte.



		\paragraph{Protocole}
        
        Nous utilisons le même protocole que celui présenté dans la partie \ref{protocole} du chapitre précédent, à savoir le modèle \textit{Topic+Influence} avec les trois thématiques \textit{Politique}, \textit{Religion} et \textit{Science}, et ce pour les trois bases de données collectées. 
        %L'algorithme \texttt{HiddenLinUCB-Sample} étant très coûteux, du fait qu’il doive échantillonner de nombreuses variables aléatoires et ceci un grand nombre de fois à chaque itération nous l'avons implémenté uniquement pour la base de données \textit{Politique}.
        Nous verrons que dans ce cas les résultats ne sont pas aussi tranchés que pour les données simulées. Nous comparons les politiques \texttt{HiddenLinUCB-Mean} et \texttt{HiddenLinUCB-Sample} à tous les algorithmes testés jusqu'ici, à savoir \texttt{CUCB}, \texttt{CUCBV}, \texttt{UCB}-$\delta$, \texttt{MOSS} et \texttt{SampLinUCB}. On fixe $L=50$ et $\alpha=\alpha_{1}=\alpha_{2}=1.96$. Nous choisissons de diviser un jour en $M \in \left\{1,2,4,8 \right\}$ périodes afin de prendre en compte l'activité des comptes selon les moments de la journée. Etant donné qu'une itération du processus d'écoute dure ici 100 secondes on a $nbStepsPerPeriod=60*60*24/M/100=108$. Finalement, pour les algorithmes nécessitant un processus de génération de l'ensemble $\mathcal{O}_{t}$, c'est-à-dire \texttt{SampLinUCB}, \texttt{HiddenLinUCB-Mean} et \texttt{HiddenLinUCB-Sample} on simule le processus pour différents $p\in \left\{0, 0.01,0.05, 0.1, 0.5,1 \right\}$, $p=0$ correspondant au cas 3 et $p=1$ au cas 1. Notons que lorsqu’ un utilisateur $i$ est dans $\mathcal{O}_{t}$, la même valeur de $x_{i,t}$ est délivrée à ces trois algorithmes, la différence se situe dans la manière dont ils s'en servent dans leur politique de sélection. 
        
        
    	\paragraph{Résultats}
        
        
Le nombre d'algorithmes et de configurations étant élevé, la représentation graphique de l'évolution de la récompense cumulée en fonction du temps sur une même courbe n'est pas envisageable. Nous proposons plutôt une représentation condensée dans laquelle, pour chaque algorithme on illustre la valeur finale de la récompense cumulée. Ainsi les figures \ref{fig:finalRewardDBUS}, \ref{fig:finalRewardDBOG} et \ref{fig:finalRewardDBBrexit} représentent cette grandeur respectivement pour les bases \textit{USElections}, \textit{OlympicGames} et \textit{Brexit} et pour les trois thématiques. Pour plus de lisibilité, nous utilisons une même couleur pour représenter les algorithmes dans lesquels la probabilité $p$ est la même. Premièrement, lorsque chaque contexte est observable ($p=1$), notre approche contextuelle (que ce soit \texttt{HiddenLinUCB-Sample} ou \texttt{HiddenLinUCB-Mean}) correspond à un algorithme  \texttt{LinUCB} classique et fonctionne mieux que les approches \texttt{CUCB}, \texttt{CUCBV}, \texttt{MOSSS} et \texttt{UCB}-$\delta$. Ce résultat montre que nous sommes en mesure de mieux anticiper les utilisateurs qui vont être les plus pertinents à l'étape suivante, compte tenu de leur activité juste avant. Cela confirme aussi le comportement non stationnaire des utilisateurs. Par exemple, les utilisateurs peuvent parler de science au cours de la journée tout en étant plus axés sur le sport quand ils reviennent à la maison. Considérer les contextes permet également de converger plus rapidement vers les utilisateurs intéressants puisque tous les comptes partagent le même paramètre $\beta$. En outre, les résultats montrent que, même pour de faibles probabilités d'observation des contextes $p$, notre politique contextuelle se comporte beaucoup mieux que les approches non contextuelles, ce qui valide empiriquement notre approche : il est possible de tirer parti de l'information contextuelle, même si une grande partie de cette information est cachée. En donnant la possibilité de sélectionner des utilisateurs même si leur contexte est inconnu, nous permettons à l'algorithme de compléter sa sélection en choisissant les utilisateurs dont le contexte moyen correspond à un profil appris. Si aucun utilisateur dans $\mathcal{O}_{t} $ ne semble actuellement pertinent, l'algorithme peut alors compter sur les utilisateurs avec une bonne qualité intrinsèque moyenne. A titre d'exemple, pour la base \textit{USElections} et la thématique science, le nombre moyen d'utilisateurs sélectionnés pour lesquels le contexte a été observé à chaque pas de temps est de 43 pour $p=0.1$ et 58 pour $p=0.5$, ce qui confirme que l'utilisation de contextes intéressants lorsque ceux-ci sont disponibles, tout en conservant une probabilité de sélection non négligeable pour les utilisateurs de qualité dont le contexte n'est pas connu. On remarque aussi que pour une même valeur de $p$, l'algorithme \texttt{HiddenLinUCB-Sample} est très souvent plus performant quand le nombre de périodes $M$ est élevé (surtout sur les bases \textit{USElections} et \textit{Brexit}). Ainsi, découper une journée en différentes périodes, dans lesquelles les utilisateurs peuvent avoir une activité plus ou moins forte, semble pertinent. En revanche, contrairement au cas des données simulées, l'approche \texttt{HiddenLinUCB-Sample} ne parvient pas à surpasser \texttt{HiddenLinUCB-Mean}. Au mieux, lorsque $M=8$, les performances sont équivalentes pour la base de données \textit{USElections}. Nous expliquons cela par le fait que dans un scénario réel, les récompenses ne suivent pas assez bien les hypothèses du modèle pour que l'échantillonnage des contextes soit suffisamment proche de la réalité, tandis que l'utilisation directe de la moyenne empirique (comme dans \texttt{HiddenLinUCB-Mean}), permet de discriminer plus efficacement les comptes les moins actifs. Un autre point important est que lorqsue $p=0$, l'algorithme \texttt{HiddenLinUCB-Sample} peut être bon que des approches de bandit stochastique de base, ce qui est dû à une mauvaise exploration de l'espace. En effet, si dans \texttt{HiddenLinUCB-Mean}, un bonus est donné aux utilisateurs peu observés (terme en $1/\sqrt{n_{i,t-1}}$), dans \texttt{HiddenLinUCB-Mean} rien ne favorise ces derniers, ce qui peut conduire à des situations ou certains comptes sont oubliés. 
Continuons cette analyse par une comparaison plus précise avec la méthode \texttt{SampLinUCB} du chapitre précédent, basée sur l'estimation des profils des utilisateurs. Nous insistons au passage sur le fait que cette approche utilise les mêmes vecteurs $x_{i,t}$ dans son processus de sélection mais s'en sert différemment. Il apparaît que pour une même valeur de $p$, les méthodes proposées dans ce chapitre - que ce soit \texttt{HiddenLinUCB-Mean} ou \texttt{HiddenLinUCB-Sample} - permet d'obtenir de meilleurs résultats, du moins pour les bases de données \textit{USElections} et \textit{Brexit} (pour la base \textit{OlympicGames}, les résultats sont plus mitigés). Ceci peut s'expliquer par le fait que l'approche de ce chapitre, bien que modélisant un terme stationnaire de biais, est essentiellement non stationnaire, à la différence de l'approche du chapitre précédent. Il semble que ceci soit particulièrement pertinent dans un réseau social puisque les utilisateurs y ont une attitude très variable de façon générale, pouvant être mieux captée par le modèle contextuel utilisé. A nouveau, lorsque $p=0$, on remarque que \texttt{HiddenLinUCB-Sample} est moins performant que \texttt{SampLinUCB}.  


                
             \begin{figureth}
		\begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBUS_PoliticFinalRwd.pdf}
			\caption{Politique}
		\end{subfigureth}
		\begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBUS_ReligionFinalRwd.pdf}
			\caption{Religion}
		\end{subfigureth}
        \begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBUS_ScienceFinalRwd.pdf}
			\caption{Science}
		\end{subfigureth}
		\caption[Récompense finale pour tous les algorithmes testés sur la base \textit{USElections}.]{Récompense finale pour tous les algorithmes testés sur la base \textit{USElections} et le modèle \textit{Topic+Influence} avec différentes thématiques.}	
			\label{fig:finalRewardDBUS}
				\end{figureth}
                
                           \begin{figureth}
		\begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBOG_PoliticFinalRwd.pdf}
			\caption{Politique}
		\end{subfigureth}
		\begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBOG_ReligionFinalRwd.pdf}
			\caption{Religion}
		\end{subfigureth}
        \begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBOG_ScienceFinalRwd.pdf}
			\caption{Science}
		\end{subfigureth}
		\caption[Récompense finale pour tous les algorithmes testés sur la base \textit{OlympicGames}.]{Récompense finale pour tous les algorithmes testés sur la base \textit{OlympicGames} et le modèle \textit{Topic+Influence} avec différentes thématiques.}	
			\label{fig:finalRewardDBOG}
				\end{figureth}


           \begin{figureth}
		\begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBBrexit_PoliticFinalRwd.pdf}
			\caption{Politique}
		\end{subfigureth}
		\begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBBrexit_ReligionFinalRwd.pdf}
			\caption{Religion}
		\end{subfigureth}
        \begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBBrexit_ScienceFinalRwd.pdf}
			\caption{Science}
		\end{subfigureth}
		\caption[Récompense finale pour tous les algorithmes testés sur la base \textit{Brexit}.]{Récompense finale pour tous les algorithmes testés sur la base \textit{Brexit} et le modèle \textit{Topic+Influence} avec différentes thématiques.}	
			\label{fig:finalRewardDBBrexit}
				\end{figureth}


        
 \textbf{Note sur l'activité des profils: }Pour chaque jeu de données, nous calculons la probabilité (a posteriori) d'être actif de chaque utilisateur, indépendamment de la récompense, pour chacune des huit périodes considérées. Concrètement, cela correspond à la valeur $p_{i,j,T}$ calculée par  \texttt{HiddenLinUCB-Sample} lorsque $p=1$ pour chaque utilisateur $i\in \mathcal{K}$ et chaque période $j\in \left\{1,...,8\right\}$. Ensuite pour chaque compte $i$, nous calculons la période $p_{i}^{\star}$ pour laquelle il a la plus forte probabilité de parler, c'est à dire $p_{i}^{\star}=\max\limits_{j\in \left\{1,...,8\right\}} p_{i,j,T}$ (on note la période correspondante $j_{i}^{\star}=\argmax\limits_{j\in \left\{1,...,8\right\}} p_{i,j,T}$). Finalement pour chaque période $j$, nous notons $q_{j}$ le nombre d'utilisateurs pour lesquels $j_{i}^{\star}=j$. La figure \ref{fig:probaTalk} représente  $q_{j}$ pour chaque période $j$ et pour les trois jeux de données, où l'on a normalisé chaque valeur par le nombre total de comptes. Ces figures permettent d'illustrer de façon synthétique le fait tous les utilisateurs ne sont pas actifs au même moment d'une part, et d'autre part que leur activité n'est pas répartie de façon uniforme. En effet si c'était le cas, on n'observerait qu'une barre différente de zéro dans le premier cas et huit barres de tailles égales dans le second. Remarquons également que pour chaque base de données, la répartition est différente. 


             \begin{figureth}
		\begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBUS_ProbaTalk.pdf}
			\caption{Base de données \textit{USElections}}
		\end{subfigureth}
		\begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBOG_ProbaTalk.pdf}
			\caption{Base de données \textit{OlympicGames}}
		\end{subfigureth}
        \begin{subfigureth}{0.5\textwidth}
			\includegraphics[width=\linewidth]{DBBrexit_ProbaTalk.pdf}
			\caption{Base de données \textit{Brexit}}
		\end{subfigureth}
		\caption[Activité des utilisateurs selon la période considérée]{Activité des utilisateurs en fonction de la période.}	
			\label{fig:probaTalk}
	\end{figureth}
        
        
        
		
\subsubsection{En ligne}

			\paragraph{Protocole}

Nous considérons notre tâche de collecte dans une expérimentation en ligne sur Twitter prenant en compte l'ensemble du réseau social ainsi que les contraintes des différentes API. Comme nous l'avons déjà présenté, l'API \textit{Follow} \textit{Streaming} de Twitter nous offre la possibilité d'écouter un total de 5000 utilisateurs du réseau social simultanément. À l'instar de l'expérimentation en ligne du chapitre \ref{FormalisationTache}, nous utiliserons cette dernière pour récupérer les contenus produits par les comptes dans $\mathcal{K}_{t}$. Dans le cas où l'on ne dispose d'aucune autre source d'information, cette API sert également à récupérer les contextes de certains utilisateurs, ce qui correspond au scénario où $\mathcal{O}_{t}=\mathcal{K}_{t-1}$. Comme nous l'avons vu dans les expérimentations hors-ligne, de façon générale, l'augmentation du nombre de contextes visibles à chaque itération permet d'améliorer les résultats. Dans cette optique, rendre disponible plus de contextes semble être pertinent. En plus des 5000 comptes que l'on peut écouter en même temps, Twitter propose également une API \textit{Sample} \textit{streaming}, qui renvoie en temps réel 1\% de tous les tweets publics. Les éléments renvoyés par cette API sont les mêmes, peu importe la connexion utilisée. Ainsi, multiplier les comptes pour récupérer plus de données via cette API est inutile. Nous utilisons cette dernière pour découvrir de nouveaux utilisateurs, mais aussi pour récolter les contextes (activités) d'un grand nombre d'utilisateurs actifs à un moment donné. Concrètement, l'utilisation de cette seconde source d'information nous permet d'avoir plus d'utilisateurs dans $\mathcal{O}_{t}$ à chaque itération. Afin d'expliciter le fonctionnement du processus de collecte en temps réel dans ce cas, nous proposons une illustration dans la figure \ref{fig:processLiveCtxt}, où trois itérations sont représentées. Au début de chaque étape, la politique de sélection des sources choisit un ensemble d’utilisateurs à suivre ($\mathcal{K}_{t}$) parmi tous les utilisateurs connus du système (${\cal K}$), selon des observations et des connaissances fournies par un module d'apprentissage correspondant à la politique en question. Ensuite, les messages postés par les $k=5000$ profils sélectionnés sont collectés via l'API \textit{Follow streaming}. Comme nous pouvons le voir dans la partie centrale du schéma, après avoir suivi les utilisateurs de $\mathcal{K}_t$ pendant l'itération courante $t$, les messages collectés sont analysés (soit par un humain, soit automatiquement) et le résultat - traduisant la pertinence - est renvoyé au module d'apprentissage. En parallèle, à chaque itération, l'activité courante de certains utilisateurs est capturée par l'API \textit{Sample streaming}. Cela nous offre la possibilité d'enrichir la base des utilisateurs potentiels ${\cal K}$, mais aussi de construire l'ensemble  des utilisateurs dont on connaît le contexte. Chaque profil ayant publié au moins un message parmi ceux qui ont été collectés avec l'API \textit{Sample streaming} à l'étape $t$ sont inclus dans $\mathcal{O}_{t+1}$, les messages d'un même auteur $i$ étant concaténés pour former $x_{i,t+1}$. À cet ensemble sont ajoutés les utilisateurs de $\mathcal{K}_{t}$, puisque leur activité complète a été suivie pendant l'étape $t$.

\begin{figureth}
			\includegraphics[width=0.8\linewidth]{taskLast.pdf}
			\caption[Illustration du système]{Illustration du système.}		
			\label{fig:processLiveCtxt}
\end{figureth}


Dans cette expérience, on fixe la durée d'une période d'écoute, notée $\mathcal{L}$, à $\mathcal{L}=15 minutes$ et l'horizon à deux semaines, ce qui correspond à $T=1344$. Nous choisissons la fonction de récompense \textit{Topic+Influence} avec la thématique politique. Comme précédemment, compte tenu des restrictions de Twitter, chaque expérience nécessite un compte développeur, ce qui limite le nombre de politiques que nous pouvons tester en parallèle. Nous avons choisi de tester les quatre stratégies suivantes : notre approche contextuelle \texttt{HiddenLinUCB-Mean}, l'algorithme \texttt{CUCBV}, une politique \texttt{Random} et une autre appelée \texttt{Static}, qui suit les mêmes 5000 comptes, sélectionnés a priori, à chaque étape du processus. Les 5000 comptes suivis par l'approche \texttt{Static} ont été choisis en sélectionnant les 5000 utilisateurs ayant cumulé le plus fort volume de récompenses selon les messages collectés par l'API \textit{Sample} sur une période de 24 heures. Pour information, certains comptes célèbres tels que \textit{@dailytelegraph}, \textit{@Independent} ou \textit{@CNBC} en faisaient partie. Remarquons enfin que $p$, la probabilité pour chaque utilisateur de révéler son activité n'est pas un paramètre, mais est contraint par la tâche. Précisons finalement que nous n'avons pas implémenté la politique \texttt{HiddenLinUCB-Sample} à cause de sa trop forte consommation en ressource (mémoire et calculatoire), en particulier dans un cadre où le nombre total de comptes peut être très grand.


			\paragraph{Algorithme détaillé}


L'implémentation de l'algorithme \texttt{HiddenLinUCB-Mean} dans ce cadre nécessite quelques adaptations par rapport au cadre générique dans lequel nous l'avons décrit. En particulier, la manipulation des différents ensembles d'utilisateurs en jeu peut s'avérer délicate. On propose ainsi de détailler le processus de collecte dans l'algorithme \ref{algoCollectLiveContext}, dont le fonctionnement général est le suivant :

Les ensembles et paramètres manipulés sont tout d'abord initialisés de la manière suivante:
\begin{itemize}
\item $V$ par une matrice identité de taille $d\times d$ et $b$ par un vecteur nul de taille $d$, avec $d$ la taille des vecteurs de contexte;
\item $\mathcal{K}$ par l'ensemble vide;
\item  $\mathcal{O}_{1}$ par les utilisateurs auteurs de messages collectés au cours d'une première utilisation de l'API \textit{Sample} pendant une période de temps d'une durée ${\cal L}$. La représentation des messages de ces utilisateurs $i \in \mathcal{O}_{1}$ correspond à leur contexte $x_{i,1}$.
\end{itemize}

L'algorithme  procède ensuite, pour chaque itération $t$ de la collecte selon:

\begin{enumerate}
\item Insertion dans $\mathcal{K}$ de chaque utilisateur de $\mathcal{O}_{t}$ n'en faisant pas encore partie  (en limitant le nombre de nouveaux entrants à  $newMax$ utilisateurs par itération afin d'éviter une sur exploration pour le cas des très grands réseaux tel que Twitter);
\item Mise à jour des moyennes empiriques des contextes $\hat{x}_{i}$ pour les profils de $\mathcal{O}_{t}$;
\item Calcul de l'estimateur du paramètre $\bar{\beta}$ ;
\item Calcul des scores de sélection $s_{i,t}$  de tous les utilisateurs dans $\mathcal{K}$ selon que leur contexte est disponible ou non. Le score des nouveaux utilisateurs est fixé à $+\infty$ pour forcer le système à les choisir une première fois. Bien que cette initialisation ne soit pas obligatoire, cela nous permet en pratique d'avoir un premier estimateur de la qualité intrinsèque de chaque utilisateur; 
\item Sélection des $k$ profils ayant les meilleurs scores  $s_{i,t}$;
\item Capture simultanée via les APIs \textit{Sample} et \textit{Follow} pendant une période de durée ${\cal L}$. L'API \textit{Follow} écoute les $k$ utilisateurs sélectionnés $\mathcal{K}_{t}$;
\item Calcul des récompenses des messages collectés pour les utilisateurs de $\mathcal{K}_t$ à partir de l'API \textit{Follow}, puis mise à jour des paramètres du modèle;
\item Mise à jour de l'ensemble des utilisateurs observés $\mathcal{O}_{t+1}$, et des contextes associés, en considérant tous les utilisateurs pour lesquels au moins un message a été collecté pendant l'itération $t$ (provenant soit de l'API \textit{Sample} soit de l'API \textit{Follow});
\end{enumerate}


\begin{algorithm}[p]
\scriptsize
 \KwIn{$k$, $T$, $\alpha$,$\alpha_{1}$,$\alpha_{2}$, ${\cal L}$, $maxNew$}
 $V = I_{d\times d}$ (matrice identité de taille $d$)\;
 $b = 0_{d}$ (vecteur de 0 de dimension $d$)\;
 $\mathcal{K} = \emptyset$\; 

$\Omega_1 = $ Données collectées depuis l'API \textit{Sample} pendant une période de  ${\cal L}$\; 
$\mathcal{O}_{1} = $ Auteurs ayant au moins un message dans $\Omega_1$\; 
\For{$t  \gets 1$ \KwTo $T$} {
	
	$nbNew=0$\; 
	\For{$i  \in \mathcal{O}_{t}$}{ 
		
		\If{$i \notin \mathcal{K}$ \textbf{et} $nbNew < maxNew$} {   \label{addPoolBeginLive}
			$nbNew = nbNew +1$\;
			$\mathcal{K} = \mathcal{K} \cup \{i\}$\; 
			$T_{i}= 0$; $n_{i}= 0$; $s_{i}= 0$; $b_{i}= 0_d$\; 
			$\bar{\mu}_{i}= 0$; $\bar{x}_{i}= 0_d$; $\hat{x}_{i}= 0_d$\;
		}    \label{addPoolEnd}
		\If{$a \in \mathcal{K}$}{ \label{observeContextBeginLive}
			Observer le contexte $x_{i,t}$ dans $\Omega_t \cup \Psi_t$\;
			Mettre à jour $\hat{x}_{i}$;
			$n_{i}= n_{i}+1$\;
		} \label{observeContextEnd}
	}
	

	$\bar{\beta} = V^{-1}b$\;  \label{updateBetaLive}
	
	\For{$i  \in \mathcal{K}$} { \label{ComputeScoresBeginLive}
   	\If{$T_{i}>0$}{
			\If{$i \in \mathcal{O}_{t}$} {
				$s_{i,t}=\bar{\mu}_{i}+(x_{i,t}-\bar{x}_{i})^{\top}\bar{\beta} + \alpha\sqrt{\dfrac{1}{N_{i}+1}+(x_{i,t}-\bar{x}_{i})^{\top}V^{-1}(x_{i,t}-\bar{x}_{i})}$\;
				}
				\Else{
 			$s_{i,t}=\bar{\mu}_{i}+(\hat{x}_{i}-\bar{x}_{i})^{\top}\bar{\beta} +\alpha_{1}\sqrt{\dfrac{1}{N_{i}+1}+(\hat{x}_{i}-\bar{x}_{i})^{\top}V^{-1}(\hat{x}_{i}-\bar{x}_{i})} +  \alpha_{2}\sqrt{\dfrac{1}{n_{i}}}$\;
				}
	
			}
			\Else{
				$s_{i,t}=\infty$;
			}
	} \label{ComputeScoresEndLive}

		$\mathcal{K}_{t} = \argmax\limits_{\hat{\mathcal{K}} \subseteq \mathcal{K}, |\hat{\mathcal{K}}|=k} \quad \sum\limits_{i \in \hat{\mathcal{K}}} s_{i,t}$ \; \label{userSelectionLive}

	\textbf{pendant} une période de ${\cal L}$ : \\ \label{collectionBeginLive}
	$\quad \quad \Omega_{t} = $ Collecter les données via l'API \textit{Sample} \; 
	$\quad \quad \Psi_{t} = $ Collecter les données via l'API \textit{Follow} centrées sur les utilsaiteurs de $\mathcal{K}_{t}$ \; 
		\For{$i  \in \mathcal{K}_t$} { \label{updateCountsBeginLive}
		Calculer $r_{i,t}$ pour $\Psi_t$\;
		\If{$i\in \mathcal{O}_{t}$}{
			$V= V+b_{i}b_{i}^{\top}/(N_{i}+1)$\;
			$b= b+b_{i}s_{i}/(N_{i}+1)$\;
			$N_{i}= N_{i}+1$\;
			$s_{i}= s_{i}+r_{i,t}$\;
            $\bar{\mu}_{i} = s_{i}/(N_{i}+1)$\;
			$b_{i}= b_{i}+x_{i,t}$\;
            $\bar{x}_{i}= b_{i}/(N_{i}+1)$\;
			$V= V+x_{i,t}x_{i,t}^{\top}-b_{i}b_{i}^{\top}/(N_{i}+1)$\;
			$V= b+r_{i,t}x_{i,t}-b_{i}s_{i}/(N_{i}+1)$
		}
	  } \label{updateCountsEndLive}
		$\Omega_{t+1} = \Omega_t$;  $\Psi_{t+1} =  \Psi_t$ \;
		$\mathcal{O}_{t+1} = $ Auteurs ayant au moins un message dans $\Omega_{t+1} \cup \Psi_{t+1}$\; \label{updateObservedUsersSetLive}
	}
\caption{Algorithme de collecte de données \texttt{HiddenLinUCB-Mean} adapté pour  l'expérience en ligne.}
\label{algoCollectLiveContext}
\end{algorithm}




			\paragraph{Résultats}


La partie gauche de la figure \ref{fig:liveContextPolitic} représente l'évolution du gain cumulé en fonction du temps (représenté en termes de nombre d'itérations). On remarque le très bon comportement de notre algorithme dans un scénario réel, car la somme des récompenses qu'il accumule croît beaucoup plus rapidement que celle des autres politiques, surtout après les 500 premières itérations. Après ces premières itérations, notre algorithme semble avoir acquis une bonne connaissance sur les distributions de récompenses en fonction des contextes observés sur les différents utilisateurs du réseau. Afin d'analyser le comportement des politiques expérimentées pendant les premières itérations de la capture, nous représentons aussi à droite de la figure \ref{fig:liveContextPolitic} un zoom des mêmes courbes sur les 150 premiers pas de temps.
Au début, la politique \texttt{Static} est plus performante que toutes les autres, ce qui peut s'expliquer par deux raisons: premièrement les algorithmes de bandits utilisés ont besoin de sélectionner tous les utilisateurs au moins une fois pour initialiser les scores et deuxièmement les utilisateurs faisant partie de l'ensemble \texttt{Static} sont supposés être des sources relativement pertinentes étant donné la façon dont ils ont été choisis. Vers l'itération 80, aussi bien l'algorithme \texttt{CUCBV} que l'algorithme contextuel deviennent meilleurs que \texttt{Static}, ce qui correspond au moment où ils  commencent à pouvoir exploiter de ``bons'' comptes identifiés. Ensuite, une période d'environ 60 itérations est observée (approximativement entre les itérations 80 et 140), au cours de laquelle l'algorithme \texttt{CUCBV} et notre approche contextuelle ont des performances comparables. Cette période s'explique par le fait que notre approche nécessite un certain nombre d'itérations pour apprendre des corrélations efficaces entre contextes et récompenses afin d'en tirer avantage. Enfin, après cette période d'initialisation, on peut remarquer un changement significatif de pente pour la courbe correspondant à notre algorithme, ce qui souligne sa faculté à être bien plus réactif dans un environnement dynamique. De plus, le volume de récompenses collectées avec notre approche sur la période d'expérimentation représente plus du double de ce qui a été collecté avec l'approche état de l'art \texttt{CUCBV}. Enfin, il est à noter que le nombre de fois que chaque utilisateur a été sélectionné par notre algorithme est mieux réparti qu'avec un algorithme stationnaire comme \texttt{CUCBV}, ce qui confirme la pertinence d'adopter une approche dynamique. En conclusion, que ce soit en ligne ou hors ligne, notre approche se révèle très efficace pour la sélection dynamique d'utilisateurs pour la collecte de données ciblée.


             \begin{figureth}
		\begin{subfigureth}{0.45\textwidth}
			\includegraphics[width=\linewidth]{liveHybridk5000T900RwdRT.pdf}
			\caption{Récompense cumulée sur toute la durée de la collecte.}
		\end{subfigureth}
		\begin{subfigureth}{0.45\textwidth}
			\includegraphics[width=\linewidth]{liveHybridk5000T900RwdRTZoom.pdf}
			\caption{Agrandissement sur les 150 premiers pas de temps.}
		\end{subfigureth}
		\caption[Récompense cumulée en fonction du temps dans l'expérience en ligne]{Récompense cumulée en fonction du temps dans l'expérience en ligne pour différentes politiques. A gauche se trouve une version agrandie des 150 premiers pas de temps.}	
			\label{fig:liveContextPolitic}
				\end{figureth}






\section{Conclusion}



Dans ce chapitre, nous avons formalisé notre tâche de collecte de données sur les réseaux sociaux comme une instance spécifique du problème de bandit contextuel, dans laquelle, à cause des restrictions imposées par les médias sociaux, seule une partie des contextes est observable à chaque itération. Pour résoudre cette tâche, nous avons proposé une adaptation de l'algorithme de bandit contextuel \texttt{LinUCB} pour le cas où certains contextes sont cachés. 

Dans le chapitre qui suit, nous introduisons un modèle dans lequel nous modélisons des relations temporelles entre les différents utilisateurs.

==> Glossaire.tex <==
\newglossaryentry{alpha}{
  type=notation,
  name={\ensuremath{\alpha}},
  description={Angle de d'attaque de la molette},
  sort={alpha}%
}

\newglossaryentry{gamma}{
  type=notation,
  name={\ensuremath{\gamma}},
  description={Angle de dépouille de la molette},
  sort={gamma}
}


